Exact-$2$-Relation Graphs

Pairwise compatibility graphs (PCGs) with non-negative integer edge weights recently have been used to describe rare evolutionary events and scenarios with horizontal gene transfer. Here we consider the case that vertices are separated by exactly two discrete events: Given a tree $T$ with leaf set $L$ and edge-weights $\lambda: E(T)\to\mathbb{N}_0$, the non-negative integer pairwise compatibility graph $\textrm{nniPCG}(T,\lambda,2,2)$ has vertex set $L$ and $xy$ is an edge whenever the sum of the non-negative integer weights along the unique path from $x$ to $y$ in $T$ equals $2$. A graph $G$ has a representation as $\textrm{nniPCG}(T,\lambda,2,2)$ if and only if its point-determining quotient $G/\!\rthin$ is a block graph, where two vertices are in relation $\rthin$ if they have the same neighborhood in $G$. If $G$ is of this type, a labeled tree $(T,\lambda)$ explaining $G$ can be constructed efficiently. In addition, we consider an oriented version of this class of graphs.

==> notes.tex <==

\newcommand{\Rkl}{\mathrel{\overset{k}{\geq}}}
\newcommand{\Rkll}{\mathrel{\overset{k+1}{\geq}}}
\newcommand{\Rkm}{\mathrel{\overset{k}{\leq}}}
\newcommand{\Rlm}{\mathrel{\overset{1}{\leq}}}
\newcommand{\Rn}{\mathrel{\overset{n}{\sim}}}
\newcommand{\Rtl}{\mathrel{\overset{2}{\geq}}}

\section{Explained by $\Rt$ instead of $\Rt/\Ro$} 

\emph{Point-determining graphs} (also known as mating-type graphs, mating graphs, M-graph or thin
graphs) are graphs in which no two vertices have the same neighborhoods. If we start with
any graph $G$, and gradually merge vertices with the same neighborhoods, we obtain a point-
determining graph, denoted by $G_{pd}$. It is easy to observe that $G_{pd}$ is always an induced subgraph of $G$. 

\TODO{define thinness relation or refer it.}

\begin{lemma} \label{lem:thin}
 For any graph $G$, $G \in G(\Rk)$ if and only if $G_{pd}$ in $G(\Rk)/\Ro$.
\end{lemma}

\begin{proof}

For a given graph $G$ such that $G_{pd}$ is in $G(\Rt/\Ro)$,
By definition there is a least resolved tree $(T,\lambda)$ explains $G_{pd}$.

Since we know the structure of $G$, we know how we get $G_{pd}$,
i.e., each vertex of $G_{pd}$ correspond to an thinness equivalent
class of vertices in $G$. We know just duplicate each leaves of $(T,\lambda)$
corresponding times, the edge labeled tree $(T',\lambda')$ explains
$G$ in $\Rt$.

On the other hand if $G \in G(\Rk)$, then there exists $(T,\lambda)$ explains $G$ with respect to $\Rk$.
Let $(T',\lambda')$ to be the edge labeled tree constructed from $(T,\lambda)$ by contracting all leaves in the same equivalent class
of $\Ro$. The edge labeling is consistant. 
Suppose $(T',\lambda')$ explains graph $H$ in $\Rk$.
We claim that $G$ and $H$ are in the same thinness equivalent class, i.e., Thus $G_{pd} = H_{pd}$.
That is because $H$ can be construced from $H$ by the contracting the corresponding vertices which was contracted in
$(T',\lambda)$. Thus $G_{pd} = H_{pd}$.

Now we claim that $G_{pd} = H_{pd}$ is in $G(\Rk)/\Ro$.

Since $H_{pd}$ is a induced subgraph of $H$, and $(T',\lambda')$ explains graph $H$ in $\Rk$.
Then the induced subtree on the leaf set of $H_{pd}$ of $(T',\lambda')$ explains graph $H_{pd}$ in $\Rk$.

\end{proof}

By Lemma~\ref{lem:thin} and Theorem~\ref{thm:block}, we immediately get the following theorem.

%\TODO{the above lemma is stronger than the following, the following is true any way.}
\begin{thm}
 $G$ is in $G(\Rt)$ if and only if the point-determining graph of $G$ is a block graph.
\end{thm}

% \TODO{the following proof can be ignored.}
% 
% \begin{proof}
%  If the point-determining graph of $G$ is a block graph $H$, then we can rebuild the tree $(T,\lambda)$, 
%  then blow up the 0-edges.
%  
%  If $G$ is in $G(\Rt)$, and there is a least resolved tree $(T,\lambda)$ explains it. 
%  Suppose $(T,\lambda)$ explain $H$ in $\Rt/\Ro$.
%  Then $G$ and $H$ are in the same thinness equivalent class. 
%  Thus the point-determining graph of $G$ is isomorphic to the point-determining graph of $G$, 
%  We know $H$ is a block graph and the point-determining graph of a block graph is also
%  a block graph, thus the point-determining graph of $G$ is a block graph.
%  
%  \end{proof}

 However the reconstruction is not unique, see Figure~\ref{fig:2recon}.

\begin{figure}[htbp!]
  \begin{center}
  \includegraphics[width=0.9\textwidth]{./2recon.pdf}
  \end{center}
 \caption{Possible triples for a rooted tree}.
 % Its corresponding graph in $G(\Rtd/\Ro)$ and two different ways to reconstruct $T,\lambda$.}
  \label{fig:2recon}
\end{figure}




\section{At least $k$ relation}

At most $k$ relation $\Rkm$ on two set $X\times X$ is the union of exactly $n$ relation for $0\leq n \leq k$.
And at least $k$ relation is $X\times X \setminus \Rkm$.


Two vertices $u$, $v$ that have the same neighbors are called \emph{twins}. 
They are called \emph{true twins} 
if they are also connected. 
Twins and true twins plays an important role in Algorithms like MO and  FPT algorithms

X is a \emph{module} if all members of $X$ have the same set of neighbors among vertices not in $X$, i.e.,
any two elements of $X$ are twins.

X is \emph{true module} if any two elements of $X$ are true twins.


modular partitions of $V$ where each partition class is a module are of particular interest.
Suppose $P$ is a modular partition. Since the partition classes are disjoint, their adjacencies
constitute a new graph, a quotient graph $G/P$, whose vertices are the members of $P$. 
That is, each vertex of 
$G/P$ is a module of $G$, 
and the adjacencies of these modules are the edges of $G/P$.

If $P$ is a nontrivial true modular partition, 
we define $G/P$ is a compact representation of all the edges that have endpoints in different partition classes of $P$. 

\subsection{At most 1 relation}

\begin{thm}
 $G$ is in $G(\Rkm)$ if and only if the true module decomposition of $G$ is forrest.
\end{thm}



\begin{lemma}
If the weakly point-determining graph of $G$ is forrest,  then $G$ is in $G(\Rlm)$.
\end{lemma}

\begin{proof}
 If the weakly point-determining graph $H$ of $G$ is forrest, we can reconstruct a cannonical tree $(T,\lambda)$ by algorithm
 in exactly 1 relation, and then blow-up the each weakly thinness class by 0 edges. 
 by the construction, for inner vertices of forrest, we duplicate, for leave vertices of forrest, we add an 0-edge and then 
 duplicate it. We claim that $(T,\lambda)$ explains $G$ with respect to $\Rlm$.
 \TODO{write a algorithm}
\end{proof}

\begin{lemma}
If $G$ is in $G(\Rlm)$, then the weakly point-determining graph  of $G$ is forrest.
\end{lemma}

\begin{proof}
If $G$ is in $G(\Rlm)$, then there is a cannonical tree $(T,\lambda)$ explains $G$ with respect to  $\Rlm$.
We consider the weakly thinness relation induced by $x,y$ if and only if $path x, y =0$.

It is indeed a weakly thinness relation.

It is in the same class as , so it is a forrest. 
\end{proof}





\TODO{maybe it is easier to define by thinness}


We say $G$ is a \emph{weekly thin} graph if $G$ has only trivial weekly thin equivalent class.


\begin{lemma}
 If $G$ is a weakly thin graph if and only if $G-\{e\} $ is a thin graph for all $e\in E(G)$.
\end{lemma}



\begin{proof}
If $G$ is a weekly thin graph, and there is an $e\in E(G)$ such that $G-\{e\}$ is not a thin graph,
i.e., there exists non-trival thinness equivalent class $R$, then $R$ is a non-trival weekly thinness equivalent class
in $G$, contradicting to the fact that $G$ is a weekly thin graph.

Suppose $G-\{e\} $ is a thin graph for all $e\in E(G)$, and suppose $G$ is not a weekly thin graph,
then there exists a non-trival weekly thinness equivalent class in $G$, say $R'$. Suppose $x,y$ are two 
distinct vertices in $R'$. Let $e=\{xy\}$. Consider $G-\{e\}$, since $x,y$ are in the same
weekly thinness equivalent class, we have $N(x)=N(y)$ in $G-\{e\}$, it contradicts to the assumption that
$G$ is a thinness class.
\end{proof}

The \emph{complement of a graph $G$}, denoted by $\overline{G}$, is a graph on the same vertices of $G$
such that two distinct vertices of $\overline{G}$ are adjacent if and only if they are not adjacent in $G$.
 
\begin{lemma}
  $G\in G(\Rkll)$ if and only if $\overline{G} \in G(\Rkm)$ if and only if the complement of weakly point-determining graph of $G$ is forrest.
 \end{lemma}


\begin{proof}
Suppose $G\in G(\Rkll)$, then by definition of  $G(\Rkll)$, $xy \in E(G)$ if and only if $d_{T,w}(x,y) \geq k+1$, further 
by definition of complement graph, $xy \in E(\overline{G})$ if and only if $d_{T,w}(x,y) \leq k$.
Thus $\overline{G} \in G(\Rkm)$.

The above process is invertible. If $\overline{G} \in G(\Rkm)$, then $xy \in E(\overline{G})$ if and only if $d_{T,w}(x,y) \leq k$, thus 
$xy \in E(G)$ if and only if $d_{T,w}(x,y) \geq k+1$, hence $G\in G(\Rkll)$.
\end{proof}

\begin{cor}
  $G\in G(\Rtl)$ if and only if $\overline{G} \in G(\Rlm)$.
 \end{cor}


\begin{algorithm} 
  \caption{Compute $(T,\lambda)$ from $(T^*,\lambda^*)$ and \TODO{weekly thin}
    classes $R_i$ with representatives $r_i\in R_i$.}
\label{alg:blow-up-true}
\begin{algorithmic}[1]
  \REQUIRE $(T^*,\lambda^*)$, $(r_i,R_i)$ for $i=1,\dots,h$. 
  \FORALL {WR-thinness classes $R_i$ with $|R_i|>1$}
     \STATE $q\leftarrow$ unique neighbor of leaf $r_i$ in $(T^*,\lambda^*)$
     \STATE remove $r_i$ from $(T^*,\lambda^*)$
           $\lambda(qq')=\lambda^*(qr_i)$ 
         \STATE insert all leaves $r\in R_i$ with edges 
           $q'r$ and $\lambda(q'r)=0$
%     \ENDIF 
  \ENDFOR
\end{algorithmic}
\end{algorithm} 








A directed version of $\Rt$ is naturally obtained by replacing $T$ with a
rooted tree and considering the ``semi-distance''
\begin{equation} 
  \vec d_{T,\lambda}(x,y) := \sum_{e\in \mathbb{P}(\lca{x,y},y)}\lambda(e)\,,
\end{equation} 
that is, the number of events on the path from the last common ancestor 
of $x$ and $y$ to $y$. We then consider the binary relation $\Rtd$ defined 
by 
\begin{equation} 
x \Rtd y \quad\textrm{if and only if}\quad \vec d_{T,\lambda}(x,y)=2
\end{equation} 
The relation $\Rtd$ naturally defines a class of directed graphs, similar
to the directed exactly-$1$-relation considered in \cite{Hellmuth:17q} and
the Fitch (directed at-least-$1$-) relation studies in \cite{Geiss:17a}.











